Sentiment Analysis of German Twitter

This thesis explores the ways by how people express their opinions on German Twitter, examines current approaches to automatic mining of these feelings, and proposes novel methods, which outperform state-of-the-art techniques. For this purpose, I introduce a new corpus of German tweets that have been manually annotated with sentiments, their targets and holders, as well as polar terms and their contextual modifiers. Using these data, I explore four major areas of sentiment research: (i) generation of sentiment lexicons, (ii) fine-grained opinion mining, (iii) message-level polarity classification, and (iv) discourse-aware sentiment analysis. In the first task, I compare three popular groups of lexicon generation methods: dictionary-, corpus-, and word-embedding-based ones, finding that dictionary-based systems generally yield better lexicons than the last two groups. Apart from this, I propose a linear projection algorithm, whose results surpass many existing automatic lexicons. Afterwords, in the second task, I examine two common approaches to automatic prediction of sentiments, sources, and targets: conditional random fields and recurrent neural networks, obtaining higher scores with the former model and improving these results even further by redefining the structure of CRF graphs. When dealing with message-level polarity classification, I juxtapose three major sentiment paradigms: lexicon-, machine-learning-, and deep-learning-based systems, and try to unite the first and last of these groups by introducing a bidirectional neural network with lexicon-based attention. Finally, in order to make the new classifier aware of discourse structure, I let it separately analyze the elementary discourse units of each microblog and infer the overall polarity of a message from the scores of its EDUs with the help of two new approaches: latent-marginalized CRFs and Recursive Dirichlet Process.

==> metadata.tex <==
% FILE: metadata.tex Version 2.1
% AUTHOR:
% Universität Duisburg-Essen, Standort Duisburg
% AG Prof. Dr. Günter Törner
% Verena Gondek, Andy Braune, Henning Kerstan
% Fachbereich Mathematik
% Lotharstr. 65., 47057 Duisburg
% entstanden im Rahmen des DFG-Projektes DissOnlineTutor
% in Zusammenarbeit mit der
% Humboldt-Universitaet zu Berlin
% AG Elektronisches Publizieren
% Joanna Rycko
% und der
% DNB - Deutsche Nationalbibliothek

%-------Eingabe der Metadaten-------------------------------------------
% Bitte füllen Sie alle Angaben aus, für die dies möglich ist. Falls
% Ihre Arbeit z.B. keinen Untertitel hat, schreiben Sie in das
% entsprechende Feld bitte ~ . Nachname und Titel  werden über ein
% zusätzliches Feld in der Schreibweise ohne Umlaute abgefragt, bitte
% lesen Sie die beigefügte Anleitung um diese korrekt auszufüllen!

%-------Daten des Autors------------------------------------------------
\Anrede{M.A.}
\Fname{Uladzimir}
\Surname{Sidarenka}
\SurnameASCII{Sidarenka}
\DOB{1984/16/06} %alle Daten bitte in 8-stelliger Schreibweise Jahr/Monat/Tag angeben
\Birthplace{Homel}

%-------Titel und Untertitel--------------------------------------------
\Type{Dissertation}
\Title{Sentiment Analysis of German Twitter}
\TitleASCII{Sentiment Analysis of German Twitter}
\Subtitle{}

%-------Eingabe der Gutachternamen--------------------------------------
\Supervisor{Prof.~Dr.~Manfred~Stede}
\GutachterA{Prof.~Dr.~Jacob~Eisenstein}
\GutachterB{Dr.~Tatjana~Scheffler}

%-------Informationen zur Universitaet----------------------------------
\Degree{Dr.~phil.}
\Fach{Linguistik}
\Faculty{Humanwissenschaftlichen Fakult\"at}
\University{Universit\"at Potsdam}
\Dekan{Prof.~Dr.~sc. Heinz  Mustermann}
\Rektor{Prof.~Dr.~Dr.~h.c. Wilhelm Muster}

%-------Pruefungsdaten: eingereicht und mdl. Pruefung-------------------
%% \SubmissionDate{2018/10/01} %alle Daten bitte in 8-stelliger Schreibweise Jahr/Monat/Tag angebe
%% \Pruefungsdatum{2018/10/01} %alle Daten bitte in 8-stelliger Schreibweise Jahr/Monat/Tag angebe
\SubmissionDate{2019/03/11}
\Pruefungsdatum{2019/07/12}

%-deutsche Schlagwoerter(bitte getrennt durch Kommata auflisten)---------------------------
\Schlagwoerter{Sentiment-Analyse, Social Media, Diskurs-Analyse}

%--englische Schlagwoerter(bitte getrennt durch Kommata auflisten)--------------------------
\Keywords{sentiment analysis, social media, discourse analysis}



